Context-aware Captions from Context-agnostic Supervision

We introduce an inference technique to produce discriminative context-aware image captions (captions that describe differences between images or visual concepts) using only generic context-agnostic training data (captions that describe a concept or an image in isolation). For example, given images and captions of "siamese cat" and "tiger cat", we generate language that describes the "siamese cat" in a way that distinguishes it from "tiger cat". Our key novelty is that we show how to do joint inference over a language model that is context-agnostic and a listener which distinguishes closely-related concepts. We first apply our technique to a justification task, namely to describe why an image contains a particular fine-grained category as opposed to another closely-related category of the CUB-200-2011 dataset. We then study discriminative image captioning to generate language that uniquely refers to one of two semantically-similar images in the COCO dataset. Evaluations with discriminative ground truth for justification and human studies for discriminative image captioning reveal that our approach outperforms baseline generative and speaker-listener approaches for discrimination.

==> sections/introduction_justify.tex <==
% Latex files for introduction to plan B "Inducing discriminative grounded language."
Language is one of the fundamental tools humans use to
communicate and represent knowledge. Importantly, it provides a
compact way to represent complex ideas, by capturing the important
aspects with a few words. In the context of machine perception, using
language to describe complex visual scene is a fundamental problem in
AI.

Importantly, capturing the key aspects of a visual scene can often depend on the
context. Consider describing an image of a bird: the attributes one might use
to describe the image might depend on the context in which we would use 
some language. In the context of birds, it might be which other bird we want
to discriminate the given bird with. In one case we may talk about the color 
of the head and in another case about the shape of the beak for others. 
Extracting the most useful language representation is best achieved 
when taking into account the some context and the context is often
about inducing discrimination between related concepts. \rama{I will add a 
figure 1 which shows this for a pair of birds.}

Unfortunately, learning to extract discrimnative language is challenging,
 since the set of combinations of classes and their
discriminative context is typically too large and one cannot hope to
experience enough samples to cover it. For instance, consider the case
of producing language to discriminate a class from a simple context
consisting of a single background class (``This is a bulldog, not a
pitbull, because...''). Even this simple case requires to cover a
quadratic number of combinations of class pairs and the set becomes
prohibitively larger when the context is more complex. Further, in some cases
the context in which we need to induce discrimination might not even be avalilabe,
say when building conversational agents, making data collection infeasible.
This is the fundamental problem we seek to address in this work: 
how can we learn to generate discriminative compact language,
given the (weak) supervision of generative language descriptions for concepts?


\begin{comment}
Consequently, we have repurposed language for various use cases, effortlessly switching between different use cases as the situation demands.
For instance, some language is literal, where the idea is to convey a concept in an accurate manner.
A good example of literal language is dictionary definitions, which use words accurately in order to communicate a concept clearly.
But how many of us speak in the manner of a dictionary?

In interpersonal communication, we often use more figurative language where the idea is to be persuasive, impactful, or effective.
For example, when explaning the difference between a horse and a zebra to a student who is confused about them, a teacher might say ``A zebra is a horse with stripes." Note that the statement might not be literally accurate (a zebra is not a horse), but the language is perhaps more \emph{effective} and might help the student learn the concept in a simpler manner.
This is a classic example of pragmatic or satisficing~\cite{} behaviour, where we forsake literal correctness for a higher objective.
Such examples are replete in our everyday life, especially in activities such as teaching, conversation, negotiation, arguments, debates etc.

Given the
foundational importance of pragmatic behaviour in human life, it is
not surprising that the study of pragmatic language has received a lot
of attention~\cite{}.
\end{comment}

The problem of generating language for some ultility or higher purpose has 
been studied in the field of {\em pragmatics}: the study of how language
 is used in practice.  Studies on pragmatic behaviour often take the shape 
 of discriminating between related concepts, implemented in the form of a reference game played
between a listener and a speaker, or generating language to refer to
one of out of a set of similar objects in an image~\cite{}.

\gal{Gal: I suggest to shorten the next two paragraphs.}
Previous work has looked at generation of pragmatic/discriminative descriptions for a variety of contexts, such as generating unambiguous referring expressions~\cite{}, where the task is to refer to an object in the image distinguishing it from other objects, modelling human behaviour in an explicit reference game played by humans~\cite{} etc. These approaches often build sophisticated language models, trained with discriminative ground truth data. However, collecting such discriminative data is a tedious, expensive and in some cases an intractable task.
For example, in some cases, the context for which pragmatic behaviour needs to emerge may not be known apriori, say in free form conversational agents.
This motivates work in derived pragmatics~\cite{}, where the task is to induce discriminative behaviour without training data.
Most previous work uses hand engineered rules to construct sentences in the derived pragmatics setting~\cite{}. A notable exception is the work by Andreas and Klein~\cite{} who induce discriminative behaviour with (weak) generative ground truth describing abstract scenes made from clipart.

Similar to Andreas and Klein, we situtate our work in the category of inducing pragmatic behaviour grounded in perception, however we are interested in inducing discriminative behaviour on real natural images as opposed to abstract scenes.
Some of our key modeling contributions are as follows.
We describe a simple, unified inference procedure to induce discriminative behaviour, which models a speaker and an introspector, in contrast to previous work which models a speaker and an external listener.
The speaker intuitively models the generative distribution, while the introspetor evaluates discriminative behaviour using the posterior of the distribution.

Using an introspection module, enables us to modify the popularly used beam search technique (used for approximate inference in sequential models) to perform approximate introspective inference and generate discriminative language.
Our entire model can be thought of as an introspecitve speaker, who generates discriminative language.
In contrast, previous work models a speaker, who generates generic or literal language and a listener who is given the sentences from the speaker and the two concepts to discriminate between and is tasked with picking discriminative sentences.
\rama{We show that our modified inference procedure is faster and leads to better discriminative outputs than a comparable filtering procedure. -- hope to have results for this.}
We then draw connections between our introspective inference objective and Maxmimum Mutual Information (MMI) training methods.
We derive an approximation to the MMI objective that is exactly equivalent to optimizing for the introspector on generative training data.
Even though we do not have discriminative ground truth to train with, we find that this procedure helps the speaker model to perform better, by making the training and inference procedures more consistent.
Indeed, we find that training the speaker leads to improvements in performance.

We apply our model to three tasks involving discriminative language generation: 1) Explaining the differences between fine grained bird categories using natural language, 2) discriminative image captioning, 3) referring expression generation. In the bird category explanation task, the goal is to explain why a given image contains one category as opposed to another. This is useful in general, since humans lack predefined notions of categories (unlike cats and dogs). We collect an evaluation dataset with 15,805 ground truth class discriminative explanations for birds corresponding to explanations of differences between 3161 pairs of semantically related birds, grounded in images, which will be made publicly available. In our second application of discriminative image captioning, the idea is to describe one image in a manner that it is unambiguous with respect to another very similar image, while in referring expression generation, we are interested in describing an object in a bounding box discriminating it with nearby boxes. We also provide proof of concept results on describing absence of concepts in images. While most image captioning efforts~\cite{} (understandably) focus on describing what is present in the image, it is often useful to describe what is not in the image. For instance, when looking for a table in a restaurant, one might say, ``there are no people at this table.'' Finally, we provide qualitative examples of our introspective speaker outputs and find that one can interpret its outputs as a `lie' in some cases, to achieve the purpose of discrimination.

Contributions:
\begin{itemize}
        \item A novel weakly-supervised introspective speaker model for discriminative language generation, where the speaker can be trained for discrimination.
        \item A demonstration of our ability to induce discriminative language with image attention on three tasks: explaining differences between birds, discriminative image captioning and referring expression generation.
        \item A new dataset with ground truth discriminative language for bird categories, to enable systematic evaluation and benchmarki	ng of future approaches on the task of weakly-supervised discriminative language generation.
        \item A first attempt at describing absence of concepts and qualitative examples hinting towards a model which `lies'.
\end{itemize}


==> sections/introduction_outline.tex <==
% Latex files for introduction to plan B "Inducing discriminative grounded language."
\noindent\textbf{Literal and Figurative Language}
\begin{itemize}
	\item Language is one of the fundamental tools of communication and exchange of ideas.
	\item Consequently, humans have evolved different uses and types of language
	\item Some language is literal, conveying a point where the idea is to convey a meaning
		induced by a series of words.
	\item Other kinds of language is more figurative, where idea is to be persuasive, or impactful or effective.
	\item Humans effortlessly switch between usage of either kind of language.
	\item For example, a teacher when explaining a child the difference between cats and dogs, might say "A cat is a dog with fur".
	\item This is a classic example of pragmatic behaviour -- the teacher in this has foresaken
		literal correctness for conveying a point persuasively.
	\item Such examples are replete in everyday life, especially in activities such as teaching, conversation, etc.
\end{itemize}

\noindent\textbf{Direct and Derived Pragmatics}
\begin{itemize}
	\item Given the foundational importance of pragmatic behaviour in human life, it is 
		unsurprising that study of pragmatic, or discriminative language received a lot of attention
	\item Discriminative or pragmatic behaviour can only be recognized as such in the presence of some context that provides grounding. 
	\item In the example of distinguishing cat and dog, the cat and the dog provide the context under which the pragmatic behaviour emerges
	\item Previous works has looked at explicitly collecting pragmatic training data for a given context, say generating referring expressions for an object in an image~\cite{}, \rama{add more examples}.
	\item These approaches fall into the category of modelling direct pragmatics, \ie by collecting ground truth pragmatic data.
	\item However, collecting such discriminative data is a tedious, expensive and in some cases intractable task.
	\item In some cases, the context for which we need to generate discriminative behaviour might not be known apriori (say in a conversation agent), which makes data collection intractable.
	\item This motivates work in derived pragmatics, which is the task of inducing discriminative language given only generative data.
	\item An excellent work of previous work in derived pragmatics is that of Andreas and Klein~\cite{} who present a neural network model for deriving pragmatic or discriminative behaviour on abstract cartoon like images.
\end{itemize}

\noindent\textbf{A model for inducing discrimination}
\begin{itemize}
	\item Similar to Andreas and Klein, we are interested in modelling discriminative (or pragmatic) language, grounded in a perceptual signal.
	\item However, our work has some key differences.
	\item We propose a novel inference scheme for inducing discriminative language, 
	\item In contrast to the approach of Andreas and Klein, our approach is conceptually simpler,
	\item While previous works employ a speaker and a listener for inducing direct or derived pragmatic behaviour, we select utterances by modelling a neural speaker and an introspector
	\item Our first contribution is in proposing a simple modification to the popularly used beam search technique, adapting it to induce class discrimination. Beam search is a popular technique commonly used for approximate inference in sequential models to select high-likelihood sentences. Our contribution is in repurposing it to pick good sentences for the speaker and introspector. 
	\item We then draw connections between our inference objective and Maxmimum Mutual Information training methods and show that the speaker model trained with MMI can understood as adapting to the introspector at inference, \emph{even} in the absence of discriminative training data.
	\item We then propose a novel attention mechanism for the speaker module which grounds discriminative language into perceptual signal.
\end{itemize}

\noindent\textbf{Applications and contributions}
\begin{itemize}
	\item We apply our model to three tasks grounded in the real world, involving discriminative language generation: 1) referring expression generation, 2) discriminative image captioning and 3) explaining the differences between fine-grained categories.
	\item Our results across human studies and evaluation against discriminative ground truth reveal our method to be better suited to generating discriminative language than competitive baselines.
	\item We draw an interesting insight, that when modelling discriminative, or in general figurative language, it might often be as useful to describe the absence of a concept, as it is to describe the presence. For instance, on looking at a table in a restaurant without people, we might say "This is a table which has no people.". Can our models do this? We also show some qualitative examples where it appears as if the model has learnt to produce a lie, \ie the model chooses to produce a non-factual statement in order to achieve the pragmatic objective.
	\item We make a simple modification to our method to generate proof-of-concept pragmatic descriptions detailing absence. Our is the first work to our knowledge to make this connection.
	\item Thus, our contributions are as follows: 1) propose a novel model for inducing discriminative (or pragmatic) language with a speaker and an introspector, the speaker in our model is trainable end to end to adapt to the introspector, 2) We show applications of our model  to three tasks: discriminative captioning, referring expression generation and explaining fine-grained category differences, 3) We provide some qualitative results on learning to describe absence and producing examples of lying-like behaviour.
\end{itemize}
\noindent\textbf{}

